An Adaptive Load Balancer For Graph Analytical Applications on GPUs

Load-balancing among the threads of a GPU for graph analytics workloads is difficult because of the irregular nature of graph applications and the high variability in vertex degrees, particularly in power-law graphs. We describe a novel load balancing scheme to address this problem. Our scheme is implemented in the IrGL compiler to allow users to generate efficient load balanced code for a GPU from high-level sequential programs. We evaluated several graph analytics applications on up to 16 distributed GPUs using IrGL to compile the code and the Gluon substrate for inter-GPU communication. Our experiments show that this scheme can achieve an average speed-up of 2.2x on inputs that suffer from severe load imbalance problems when previous state-of-the-art load-balancing schemes are used.

==> Makefile <==
TGT=paper

BIBTEX=bibtex
PDFLATEX=pdflatex

# Ignore these for now!
#PS2PDF_OPTS=-dEmbedAllFonts=true -dSubsetFonts=true -dEPSCrop=true -dPDFSETTINGS=/prepress 
#LATEX_OPTS=-interaction=nonstopmode -halt-on-error
LATEX_OPTS= -shell-escape 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"


.PHONY: all clean

all: $(TGT).pdf

$(TGT).pdf : $(TGT).tex Sections/*.tex References/*.bib figs/*.tex tables/*.tex
	$(PDFLATEX) $(LATEX_OPTS) $(TGT).tex
	@if(grep "There were undefined" $(TGT).log > /dev/null);\
	then \
		$(BIBTEX) *.aux; \
		$(PDFLATEX) $(LATEX_OPTS) $(TGT).tex; \
		$(PDFLATEX) $(LATEX_OPTS) $(TGT).tex; \
	fi
	@if(grep "Rerun" $(TGT).log > /dev/null);\
	then \
		$(PDFLATEX) $(LATEX_OPTS) $(TGT).tex;\
	fi

clean:
	rm -rf *.aux $(TGT).log $(TGT).blg $(TGT).dvi *.bbl
	rm -rf $(TGT).out $(TGT)-pics.pdf $(TGT).fdb_latexmk
	rm -rf $(TGT).pdf $(TGT).ps $(TGT).fls 
	#$(TGT).bbl



==> Sections/06_3-Results_MultiHostMultiGPU.tex <==

\begin{comment}

\subsection{Multi-Host Multi-GPUs}
Figure~\ref{fig:bridges} compares the performance of D-IrGL (ALB) with that of D-IrGL (TWC) and Lux frameworks, which support multi-host multi-GPU 
graph analytical applications, on up to 16 GPU of Bridges-Pascal. 
It is clear that D-IrGL (TWC), even without thread block load balancing support, performs better than Lux for all configurations.
D-IrGL (TWC) and D-IrGL (ALB) perform similary on uk2007 
but D-IrGL (ALB) is slightly faster than D-IrGL (TWC) on twitter40.
On rmat26 and rmat27, D-IrGL (ALB) is faster than D-IrGL (TWC) by an average speed up of \todo{$4\times$}. 

To analyze the performance improvement in rmat26 and rmat27, we show the breakdown of the total execution time
into computation and non-overlapping communication time on 16 GPUs as described in \todo{Section~\ref{sec:singleHostMultiGPUs}}.
The results show that most applications in D-IrGL (TWC) spend 
most of the execution time performing computation. 
These inputs have a very large max $D_{out}$ (shown in Table~\ref{tbl:inputs})
which makes them suffer from much more from thread block load imbalance 
on one of the GPUs, even when used on 16 GPUs.
D-IrGL (ALB) is effective in reducing the computation time on the GPUs by
balancing load across the thread blocks on each GPU to improve the
performance of the application in the multi-host multi-GPU system.

We also observe that D-IrGL (ALB) performs similar to uk2007 for all
configurations. This graph has a max $D_{out}$ of 15,402, which is less than the
number of threads launched in our system (i.e, \todo{26,624}), which is our threshold
to identify high-degree vertices. Hence, the graph does not have any
high-degree active vertex in any round of the computation. D-IrGL (ALB) helps
in minimizing the overhead at runtime by not applying thread block balancing
strategy in any round.

In summary, our adaptive load balancer (ALB) is effective in improving
performance of applications significantly on the configurations that suffer from thread block 
load imbalance in both single GPU and multi-GPU systems 
with minimal overhead on configurations that have balanced thread block load.

\end{comment}

\begin{comment}

\subsubsection{Total time comparison for async}
\subsubsection{Reduction in number of iterations for async.}

\todo{The Figure\ref{fig:multiHostMultiGPUs}} realizes the improvements by showing the breakdown of the time computation and synchronization time
breadk down for \todo{16 GPUs} for these graphs. It can be seen that thread block imbalance can severly effect computation time of GPU, as a results,
all the hosts in entire cluster bottlenecked by the straglled GPU. D-IrGL (ALB) is effective in detecting such anomolies at runtime hence improving
the overall performance of the application even under the mult-host multi-GPU configuration. 

The figure~\ref{fig:multiHostMultiGPUs} also show some improvement for twitter40, but it is also comparable to the D-IrGL for uk2007. Though uk2007 have huge variation in their degrees,
it does not suffer from huge thread block load imbalance. It is because the max out degree of the graph is \todo{XXX}, 
which is less than the number of threads (\todo{YYY}) that are lanuched by the application. Hence, it is beneficial to retain the benefits on TWC scheme
by balancing load within the thread block.
\end{comment}


